PHD-GIFs: Personalized Highlight Detection for Automatic GIF Creation

Highlight detection models are typically trained to identify cues that make visual content appealing or interesting for the general public, with the objective of reducing a video to such moments. However, the "interestingness" of a video segment or image is subjective. Thus, such highlight models provide results of limited relevance for the individual user. On the other hand, training one model per user is inefficient and requires large amounts of personal information which is typically not available. To overcome these limitations, we present a global ranking model which conditions on each particular user's interests. Rather than training one model per user, our model is personalized via its inputs, which allows it to effectively adapt its predictions, given only a few user-specific examples. To train this model, we create a large-scale dataset of users and the GIFs they created, giving us an accurate indication of their interests. Our experiments show that using the user history substantially improves the prediction accuracy. On our test set of 850 videos, our model improves the recall by 8% with respect to generic highlight detectors. Furthermore, our method proves more precise than the user-agnostic baselines even with just one person-specific example.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst


==> definitions.tex <==
% \newcommand{\indicator}[1]{\mathbbm{1}_{\left[ {#1} \right] }}


% \newcommand{\comment}[1]{}

\def\bigO2{\mbox{${\cal O}$}}
\def\bigO{O}

\def\mA{\mathcal{A}}
\def\mB{\mathcal{B}}
\def\mC{\mathcal{C}}
\def\mG{\mathcal{G}}
\def\mV{\mathcal{V}}
\def\mE{\mathcal{E}}
\def\mF{\mathcal{F}}
\def\mH{\mathcal{H}}
\def\mL{\mathcal{L}}
\def\mN{\mathcal{N}}
\def\mS{\mathcal{S}}
\def\mT{\mathcal{T}}
\def\mW{\mathcal{W}}
\def\mX{\mathcal{X}}
\def\mY{\mathcal{Y}}
\def\1n{\mathbf{1}_n}
\def\0{\mathbf{0}}
\def\1{\mathbf{1}}


\def\balpha{\boldsymbol{\alpha}}
\def\bdelta{\boldsymbol{\delta}}
\def\bzeta{\boldsymbol{\zeta}}
\def\bphi{\boldsymbol{\phi}}
\def\btau{\boldsymbol{\tau}}
\def\bmu{\boldsymbol{\mu}}
\def\bsigma{\boldsymbol{\sigma}}
\def\bSigma{{\bm \Sigma} }
\def\btheta{\boldsymbol{\theta}}
\def\bvartheta{\boldsymbol{\vartheta}}


\def\balpha{\mbox{\boldmath{$\alpha$}}}
\def\bbeta{\mbox{\boldmath{$\beta$}}}
\def\bdelta{\mbox{\boldmath{$\delta$}}}
\def\bgamma{\mbox{\boldmath{$\gamma$}}}
\def\blambda{\mbox{\boldmath{$\lambda$}}}
\def\bsigma{\mbox{\boldmath{$\sigma$}}}
\def\bomega{\mbox{\boldmath{$\omega$}}}
\def\bxi{\mbox{\boldmath{$\xi$}}}



\def\bpsi{\mbox{\boldmath $\psi $}}
\def\bone{\mbox{\bf 1}}
\def\bzero{\boldsymbol{ 0}}

\def\WB{{\bf WB}}

\def\A{{\bf A}}
\def\B{{\bf B}}
\def\C{{\bf C}}
\def\D{{\bf D}}
\def\E{{\bf E}}
\def\F{{\bf F}}
\def\G{{\bf G}}
\def\H{{\bf H}}
\def\I{{\bf I}}
\def\J{{\bf J}}
\def\K{{\bf K}}
\def\L{{\bf L}}
\def\M{{\bf M}}
\def\N{{\bf N}}
\def\O{{\bf O}}
\def\P{{\bf P}}
\def\Q{{\bf Q}}
\def\R{{\bf R}}
\def\S{{\bf S}}
\def\T{{\bf T}}
\def\U{{\bf U}}
\def\V{{\bf V}}
\def\W{{\bf W}}
\def\X{{\bf X}}
\def\Y{{\bf Y}}
\def\Z{{\bf Z}}

\def\a{{\bf a}}
\def\b{{\bf b}}
\def\c{{\bf c}}
\def\d{{\bf d}}

\def\f{{\bf f}}
\def\g{{\bf g}}
\def\h{{\bf h}}
\def\i{{\bf i}}
\def\j{{\bf j}}
\def\k{{\bf k}}
\def\l{{\bf l}}
\def\m{{\bf m}}
\def\n{{\bf n}}
\def\o{{\bf o}}
\def\p{{\bf p}}
\def\q{{\bf q}}
\def\r{{\bf r}}
\def\s{{\bf s}}
\def\t{{\bf t}}
\def\u{{\bf u}}
\def\v{{\bf v}}
\def\w{{\bf w}}
\def\x{{\bf x}}
\def\y{{\bf y}}
\def\z{{\bf z}}

\def\vbphi{\vec{\mbox{\boldmath $\phi$}}}
\def\vbtau{\vec{\mbox{\boldmath $\tau$}}}
\def\vbtheta{\vec{\mbox{\boldmath $\theta$}}}
\def\vI{\vec{\bf I}}
\def\vR{\vec{\bf R}}
\def\vV{\vec{\bf V}}

%%% Vector notation for sections 3 and 4
%%% Vector notation for sections 3 and 4
\def\mvec{\vec{m}}
\def\fvec{\vec{f}}
\def\appfvec{\vec{f}_k}
\def\avec{\vec{a}}
\def\bvec{\vec{b}}
\def\evec{\vec{e}}
\def\uvec{\vec{u}}
\def\xvec{\vec{x}}
\def\wvec{\vec{w}}
\def\gradvec{\vec{\nabla}}

\def\aM{\mbox{\bf a}_M}
\def\aS{\mbox{\bf a}_S}
\def\aO{\mbox{\bf a}_O}
\def\aL{\mbox{\bf a}_L}
\def\aP{\mbox{\bf a}_P}
\def\ai{\mbox{\bf a}_i}
\def\aj{\mbox{\bf a}_j}
\def\an{\mbox{\bf a}_n}
\def\a1{\mbox{\bf a}_1}
\def\a2{\mbox{\bf a}_2}
\def\a3{\mbox{\bf a}_3}
\def\a4{\mbox{\bf a}_4}

\def\sx{\mbox{\scriptsize\bf x}}
\def\st{\mbox{\scriptsize\bf t}}
\def\ss{\mbox{\scriptsize\bf s}}
\def\cR{{\cal R}}
\def\calD{{\cal D}}
\def\calS{{\cal S}}

\def\sigmae{\sigma}
\def\sigmam{\sigma}

\def\balpha{\boldsymbol{\alpha}}
\def\bbeta{\boldsymbol{\beta}}
\def\bdelta{\boldsymbol{\delta}}
\def\bgamma{\boldsymbol{\gamma}}
\def\blambda{\boldsymbol{\lambda}}
\def\bsigma{\boldsymbol{\sigma}}
\def\btheta{\boldsymbol{\theta}}
\def\bomega{\boldsymbol{\omega}}
\def\bxi{\boldsymbol{\xi}}

% \newcommand{\denselist}{\itemsep -1pt}
% \newcommand{\sparselist}{\itemsep 1pt}



 \newcommand{\ie}{\emph{i.e.\;}}
 \newcommand{\eg}{\emph{e.g.\;}}
 \newcommand{\etal}{\emph{et al.\;}}
 \newcommand{\etc}{\emph{etc.\;}}

 \newcommand{\cf}{\emph{c.f.\;}}


==> old_tables.tex <==
%-----------------------------------------------------------------------------
\begin{table*}[t!]
\centering
\setlength\extrarowheight{1ex}
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}[width=\textwidth]{@{}r|cc|cc|HHcc|P{11em}@{}}
&\multicolumn{2}{c}{mAP}&\multicolumn{2}{c}{MSD}&\multicolumn{2}{c}{%Precision @6
}&\multicolumn{2}{c|}{Recall @5}&\\[-1ex]
Model & \cite{Gygli17DeepCut} & 5 sec &  \cite{Gygli17DeepCut} & 5 sec & \cite{Gygli17DeepCut} & 5 sec& \cite{Gygli17DeepCut} & 5 sec& Notes\\\hline \hline
NEAT: &15.32\% & - & \textbf{42.11\%} & - & 8.69\% & - & \textbf{26.09\%} & - & \hl{Internal}\\
Random:&12.28\% & 12.97\% & 50.47\% & 50.60\% & 7.07\% & 7.06\% & 17.33\% & 21.38\% & -\\
video2gif:&12.65\% & 15.69\% & 52.80\% & 42.59\% & 6.76\% & 8.24\% & 17.45\% & 27.28\% & As in \cite{gygli2016video2gif}\\ 
%VMMR: & 12.52\% & 12.73\% & 74.62\% & 80.49\% & 7.43\% & 7.15\% & 28.46\% & 27.41\% & w/o hist, averaged sim\\
VMMR &-&-&-&-&-&-& \textbf{25.42\%} & 23.21\% & w/o hist, averaged sim\\
SVM-NPHD:& 13.96\% & 14.47\% & 47.14\% & 45.55\% & 8.14\% & 8.00\% & 22.04\% & 26.13\% & w/ perso\\
Non-PHD: & 15.30\% & 15.86\% & 43.66\% & 42.06\% & 8.38\% & 8.39\% & 23.63\% & 28.42\% & w/ perso
\\ %GridSearchNone/conc0000000000010Deep128_relu_DropOut0.68_0.44_decay0.003_lr0.00070perso /-5391
& \textbf{15.67\%} & \textbf{16.15\%} & \textbf{42.92\%} & \textbf{41.26\%} & 8.80\% & 8.73\% & 24.92\% & \textbf{28.92\%} &w/ both\\ 
%GridSearchNone/conc0000000000010Deep128_relu_DropOut0.68_0.44_decay0.003_lr0.00070both /-8386

\hline\hline
min($\{d_i\}$) & 15.43\% & 15.49\% & 44.12\% & 44.22\% & 8.17\% & 8.02\% & 27.40\% & 26.44\% & w/o training\\
%VMMR& 13.55\% & 13.89\% & 71.88\% & 76.12\% & 8.00\% & 8.06\% & 31.80\% & 31.88\% & w/ hist, averaged sim\\
VMMR &-&-&-&-&-&-& \textit{28.84\%} & 28.22\% & w/ hist, euclidean av\\
%SVM-D: & 15.20\% & 15.62\% & 44.27\% & 44.02\% & 8.21\% & 8.19\% & 27.26\% & 28.02\% & D statistics\\
SVM-AllD: & 15.23\% & 15.64\% & 44.15\% & 43.49\% & 8.34\% & 8.45\% & 27.77\% & 28.01\% & D to 20 closest\\
SVM-LateFus: %& 15.38\% & 15.70\% & 47.07\% & 45.41\% & 9.73\% & 9.74\% & 26.36\% & 30.00\% & SVM-(NPHD + AllD)\\
& 15.00\% & 15.32\% & 44.08\% & 43.26\% & 8.25\% & 8.37\% & 26.81\% & 27.09\% & SVM-NPHD + -allD, norm
\\\hline
\multicolumn{10}{c}{Late fusion of Deep models and SVM-allD: addition of normalized ([0-1]) prediction scores }\\
PHD-C* & 15.85\% & \underline{16.43\%} & 42.75\% & 40.98\% & 8.55\% & 8.64\% & 27.50\% & 30.52\% & w/ perso, norm\\
& \textit{16.08\%} & \textbf{16.49\% }& 42.07\% & 40.74\% & 8.77\% & 8.89\% & 28.22\% & \textit{31.16\%} & w/ both, norm\\
PHD-CD& 15.44\% & 16.13\% & 42.96\% & 41.49\% & 8.45\% & 8.55\% & 27.26\% & 29.11\% & w/ perso, norm\\%GridSearchCD/conc0000000000110Deep64_relu_DropOut0.60_0.34_decay0.008_lr0.00040perso /-1797
& \textbf{16.24\%} & 16.32\% & \textbf{41.78\%} & 40.57\% & 8.58\% & 8.93\% & 28.61\% & \textbf{31.37\%} & w/ both, norm\\
%GridSearchCD/conc0000000000110Deep128_relu_DropOut0.63_0.25_decay0.044_lr0.00029both /-10183
PHD-CAD& 15.62\% & 16.15\% & 42.33\% & 40.50\% & 8.59\% & 8.77\% & 28.61\% & 30.66\% &w/ perso, norm\\
%GridSearchCAD/conc0001000000110Deep512_64_relu_DropOut0.64_0.25_decay0.017_lr0.00099perso /-10183
& \underline{16.15\%} & 16.30\% & \textit{41.99\%} & \textbf{40.22\%} & 8.67\% & 8.90\% & \textbf{29.07\%} & \underline{31.22\%} &w/ both, norm\\%GridSearchCAD/conc0001000000110Deep256_32_relu_DropOut0.62_0.17_decay0.001_lr0.00058both /-4792
PHD-CA& 15.93\% & \textbf{16.49\%} & 42.14\% & \textit{40.48\%} & 8.55\% & 8.74\% & 27.76\% & 30.03\% & w/ perso, norm \\
%GridSearchCA/conc0001000000010Deep512_64_relu_DropOut0.71_0.18_decay0.001_lr0.00048perso /-4193
& 15.94\% & 16.18\% & 42.57\% & 40.89\% & 8.89\% & 8.85\% & \underline{28.89\%} & 30.07\% & w/ both, norm\\
%GridSearchCA/conc0001000000010Deep512_relu_DropOut0.73_0.16_decay0.001_lr0.00172both /-9584
%PHD-CA\_D**%& 15.66\% & 16.37\% & 41.71\% & 40.77\% & 8.58\% & 8.72\% & 32.59\% & 34.82\% & w/ perso, norm\\
%GridSearchCA_D/conc0011000000110Deep128_relu_DropOut0.69_0.18_decay0.039_lr0.00051perso /-7787
%& 15.83\% & 16.26\% & 42.27\% & 40.64\% & 8.76\% & 8.94\% & 27.68\% & 30.62\% & w/ perso, norm, allD\\
%& 15.94\% & 15.81\% & 41.58\% & 40.86\% & 8.22\% & 8.47\% & 31.57\% & 34.47\% & w/ both, norm\\%GridSearchCA_D/conc0011000000110Deep256_128_64_32_relu_DropOut0.57_0.37_decay0.005_lr0.00028both /-7188
%& 16.04\% & 16.13\% & 41.91\% & 40.58\% & 8.51\% & 8.61\% & 29.24\% & 30.71\% & w/ both, norm, allD\\

%PHD-C\_Dall& 15.54\% & 16.22\% & 42.41\% & 41.06\% & 8.49\% & 8.85\% & 31.55\% & 34.62\% & w/ perso, norm\\%GridSearchC_Dall/conc0010000001010Deep128_relu_DropOut0.68_0.44_decay0.003_lr0.00070perso /-5391
%& 16.10\% & 16.39\% & 42.28\% & 40.50\% & 8.70\% & 8.76\% & 31.43\% & 34.06\% & w/ both, norm\\%GridSearchC_Dall/conc0010000001010Deep128_relu_DropOut0.68_0.44_decay0.003_lr0.00070both /-9584
PHD-RH\_D** %& 15.93\% & 16.37\% & 41.80\% & 40.95\% & 8.74\% & 8.56\% & 32.14\% & 33.50\% & w/ perso, norm\\
%GridSearchRH_D/LSTM1000_1110100000110Deep256_64_relu_DropOut0.63_0.25_decay0.121_lr0.00015perso /-9584
& 15.71\% & 16.31\% & 42.11\% & 40.73\% & 8.71\% & 8.78\% & 27.77\% & 30.45\% & w/ perso, norm
\\
%& 15.89\% & 16.33\% & 41.85\% & 40.90\% & 8.65\% & 8.61\% & 31.82\% & 33.79\% & w/ both, norm\\%GridSearchRH_D/LSTM1000_1110100000110Deep64_32_32_32_relu_DropOut0.65_0.22_decay0.002_lr0.00084both /-5391
& 15.94\% & 16.39\% & \underline{41.95\%} & \underline{40.39\%} & 8.88\% & 8.83\% & 28.43\% & 30.81\% & w/ both, norm\\

\multicolumn{10}{l}{* same model as the NPHD above}\\[-1pt]
\multicolumn{10}{l}{** models trained with concatenating D stats which are replaced with ones at test time}
\end{tabular}
\vspace{-.5ex}
\caption{OpB. Preliminary Results (temporally segmented with \cite{Gygli17DeepCut} unless otherwise indicated). For mAP, P@6 and R@6, the higher the score, the better the method. For MSD, the smallest is better. Best result in \textbf{bold}, second \underline{underlined}, third in \textit{italics}.}
\label{tb:methodPref}
\end{table*}
%-----------------------------------------------------------------------------

%-----------------------------------------------------------------------------
\begin{table*}[t!]
\centering
\setlength\extrarowheight{1ex}
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}[width=\textwidth]{@{}r|cc|cc|HHcc|P{11em}@{}}
&\multicolumn{2}{c}{mAP}&\multicolumn{2}{c}{MSD}&\multicolumn{2}{c}{%Precision @6
}&\multicolumn{2}{c|}{Recall @6}&\\[-1ex]
Model & \cite{Gygli17DeepCut} & 5 sec &  \cite{Gygli17DeepCut} & 5 sec & \cite{Gygli17DeepCut} & 5 sec& \cite{Gygli17DeepCut} & 5 sec& Notes\\\hline \hline
NEAT: &15.32\% & - & \textbf{42.11\%} & - & 8.69\% & - & \textbf{29.53\%} & - & \hl{Internal}\\
Random:&12.28\% & 12.97\% & 50.47\% & 50.60\% & 7.07\% & 7.06\% & 20.49\% & 25.02\% & -\\
vid2gif:&12.65\% & 15.69\% & 52.80\% & 42.59\% & 6.76\% & 8.24\% & 20.72\% & 31.42\% & As in \cite{gygli2016video2gif}\\ 
%VMMR: & 12.52\% & 12.73\% & 74.62\% & 80.49\% & 7.43\% & 7.15\% & 28.46\% & 27.41\% & w/o hist, averaged sim\\
VMMR &-&-&-&-&-&-& 28.46\% & 27.41\% & w/o hist, averaged sim\\
SVM-NPHD:& 13.96\% & 14.47\% & 47.14\% & 45.55\% & 8.14\% & 8.00\% & 26.03\% & 29.60\% & w/ perso\\

Non-PHD: & 15.30\% & 15.86\% & 43.66\% & 42.06\% & 8.38\% & 8.39\% & 26.70\% & 32.79\% & w/ perso
\\ % /-5391
%& 15.24\% & \textbf{16.25\%} & 44.29\% & 42.35\% & 8.57\% & 8.52\% & 27.75\% & \textbf{33.67\%} & w/ perso\\%GridSearchNone/conc0000000000010Deep128_relu_DropOut0.68_0.44_decay0.003_lr0.00070perso /-1797
%& 15.30\% & 15.86\% & 43.66\% & 42.06\% & 8.38\% & 8.39\% & 26.70\% & 32.79\% &\\
 &\textbf{ 15.51\% }& \textbf{16.14\%} & 42.57\% & \textbf{40.69\%} & 8.92\% & 8.74\% & 28.37\% & \textbf{33.56\%} &
w/ both\\ %GridSearchNone/conc0000000000010Deep256_128_32_32_relu_DropOut0.71_0.22_decay0.005_lr0.00099both
%& 15.72\% & 16.36\% & 42.27\% & 40.66\% & 8.96\% & 8.64\% & 28.46\% & 32.89\% &

\hline 
min($\{d_i\}$) & 15.43\% & 15.49\% & 44.12\% & 44.22\% & 8.17\% & 8.02\% & 30.69\% & 30.72\% & \\
%VMMR& 13.55\% & 13.89\% & 71.88\% & 76.12\% & 8.00\% & 8.06\% & 31.80\% & 31.88\% & w/ hist, averaged sim\\
VMMR &-&-&-&-&-&-& 31.80\% & 31.88\% & w/ hist, euclidean av\\
SVM-D: & 15.20\% & 15.62\% & 44.27\% & 44.02\% & 8.21\% & 8.19\% & 30.64\% & 31.55\% & D statistics
\\
SVM-AllD: & 15.23\% & 15.64\% & 44.15\% & 43.49\% & 8.34\% & 8.45\% &\textbf{ 31.32\% }& 32.01\% & D to 20 closest\\
SVM-LateFus: & 15.38\% & 15.70\% & 47.07\% & 45.41\% & 9.73\% & 9.74\% & 26.36\% & 30.00\% & SVM-(NPHD + AllD)
\\
& 15.00\% & 15.32\% & 44.08\% & 43.26\% & 8.25\% & 8.37\% & 29.45\% & 31.18\% & same, but norm [0-1]
\\
NPHD + SVM-AllD: & 15.33\% & 16.18\% & 43.16\% & 41.10\% & 8.44\% & 8.48\% & 27.61\% & 32.75\% & w/ perso
\\
& 15.75\% & 16.02\% & 42.88\% & 41.82\% & 8.60\% & 8.86\% & 31.84\% & 33.84\% & w/ perso, norm
\\
& 15.85\% & 16.60\% & \textbf{41.79}\% & \textbf{39.88}\% & 8.96\% & 8.74\% & 29.21\% & 33.27\% &
w/ both\\
PHD-CD: & 15.16\% & 15.82\% & 43.68\% & 41.38\% & 8.92\% & 8.50\% & 27.83\% & 32.45\% &  w/ perso, w/ hist
\\%GridSearchCD/conc0000000000110Deep64_relu_DropOut0.60_0.34_decay0.008_lr0.00040perso /-1797
& 15.32\% & 16.12\% & 43.35\% & 41.13\% & 8.87\% & 8.62\% & 28.46\% & 32.97\% & w/ perso, late fus
\\
& 15.16\% & 15.83\% & 43.67\% & 41.37\% & 8.92\% & 8.52\% & 27.83\% & 32.49\% & w/ perso, w/o hist\\
& 15.70\% & 16.54\% & 42.21\% & 40.57\% & 8.74\% & 8.88\% & 28.12\% & 34.22\% & w/ both, w/ hist
\\%GridSearchCD/conc0000000000110Deep128_relu_DropOut0.63_0.25_decay0.044_lr0.00029both 
& 15.88\% & 16.65\% & 41.72\% & 39.90\% & 8.70\% & 9.04\% & 28.53\% & 34.65\% & w/ both, late fus
\\
& 15.70\% & 16.54\% & 42.21\% & 40.58\% & 8.74\% & 8.88\% & 28.12\% & 34.22\% & w/ both, w/o hist
\\

PHD-C\_Dall: & 15.27\% & 15.90\% & 43.31\% & 41.62\% & 8.65\% & 8.57\% & 27.73\% & 32.86\% & w/ perso w/ hist\\%GridSearchC_Dall/conc0010000001010Deep128_relu_DropOut0.68_0.44_decay0.003_lr0.00070perso /-5391
& 15.52\% & 16.06\% & 42.81\% & 41.03\% & 8.71\% & 8.61\% & 28.71\% & 33.18\% & NPHD + SVM-allD
\\
& 15.27\% & 15.90\% & 43.31\% & 41.62\% & 8.65\% & 8.57\% & 27.73\% & 32.86\% & w/ perso w/o hist\\
& 15.49\% & 16.38\% & 42.67\% & 40.88\% & 9.01\% & 9.00\% & 28.36\% & 34.28\% & w/ both w/ hist 
\\ %GridSearchC_Dall/conc0010000001010Deep128_relu_DropOut0.68_0.44_decay0.003_lr0.00070both /-9584
& 15.76\% & \textbf{16.66\%} & 42.11\% & \textbf{39.95\%} & 8.91\% & 8.97\% & 29.08\% & \textbf{34.73\%} &
 NPHD + SVM-allD\\
& 15.46\% & 16.35\% & 42.74\% & 40.83\% & 8.95\% & 8.98\% & 28.22\% & 34.32\% & w/ perso, w/o hist
\\

PHD-CA\_D & 15.78\% & 16.16\% & 42.78\% & 41.08\% & 8.61\% & 8.58\% & 28.85\% & 33.24\% &
w/ perso, w/ hist \\%GridSearchCA_D/conc0011000000110Deep128_relu_DropOut0.69_0.18_decay0.039_lr0.00051perso /-7787
%& 15.63\% & 16.55\% & 42.42\% & 40.74\% & 8.84\% & 9.02\% & 29.71\% & 34.95\% &\\%GridSearchCA_D/conc0011000000110Deep256_128_relu_DropOut0.77_0.42_decay0.005_lr0.00116perso 
& \textbf{15.99\%} & 16.35\% & 41.97\% & 40.54\% & 8.65\% & 8.70\% & 29.69\% & 33.70\% & PHD-CA + SVM-D
\\
& 15.66\% & 16.37\% & 41.71\% & 40.77\% & 8.58\% & 8.72\% & 32.59\% & 34.82\% &same, norm\\

& 14.97\% & 16.05\% & 44.99\% & 42.98\% & 8.34\% & 8.56\% & 27.53\% & 32.83\% & w/ perso, w/o hist
\\
& 15.76\% & 16.07\% & 42.40\% & 40.82\% & 8.65\% & 8.45\% & 29.67\% & 33.71\% & w/ both, w/ hist\\%GridSearchCA_D/conc0011000000110Deep256_128_64_32_relu_DropOut0.57_0.37_decay0.005_lr0.00028both /-7188
& 15.90\% & 16.13\% & \textbf{41.95\%} & 40.55\% & 8.66\% & 8.49\% & 30.59\% & 33.58\% &
 PHD-CA + SVM-D \\
& 15.56\% & 16.08\% & 42.88\% & 41.27\% & 8.70\% & 8.53\% & 28.54\% & 33.31\% & w/ both, w/o hist
\\

%PHD-CA_Dall & 15.45\% & 16.12\% & 42.31\% & 40.81\% & 8.77\% & 8.72\% & 29.03\% & 33.83\% w/ both, multinet &//GridSearchCA_Dall/conc0011000001010Deep128_relu_DropOut0.71_0.28_decay0.007_lr0.00048both /-8386
%& 15.57\% & 16.20\% & 41.85\% & 40.14\% & 8.85\% & 8.70\% & 29.85\% & 33.55\% & w/ both, late fusion\\
%& 15.36\% & 16.22\% & 42.98\% & 41.10\% & 8.93\% & 8.60\% & 28.76\% & 33.37\% & w/ both, w/o hist\\
%& 15.13\% & 16.29\% & 42.75\% & 40.85\% & 8.63\% & 9.00\% & 28.15\% & 33.86\% & w/ perso, multinet\\GridSearchCA_Dall/conc0011000001010Deep512_relu_DropOut0.59_0.35_decay0.003_lr0.00018perso /-5990
%& 15.11\% & 16.31\% & 42.75\% & 40.54\% & 8.49\% & 9.05\% & 27.66\% & 34.04\% & w/ perso, late fus\\
%& 13.86\% & 14.60\% & 47.09\% & 45.11\% & 7.98\% & 8.14\% & 23.97\% & 30.36\% & w/ perso, w/o hist\\



PHD-RH\_D & 15.49\% & 16.22\% & 42.46\% & 41.28\% & 8.80\% & 8.70\% & 28.93\% & 33.27\% & w/ perso, w/ hist
\\%GridSearchRH_D/LSTM1000_1110100000110Deep256_64_relu_DropOut0.63_0.25_decay0.121_lr0.00015perso /-9584
& 15.65\% & 16.28\% & 42.03\% & 40.88\% & 8.74\% & 8.70\% & 29.89\% & 33.16\% & late fus SVM-D
\\
& 15.47\% & 16.11\% & 43.07\% & 41.78\% & 8.77\% & 8.73\% & 28.88\% & 33.86\% &
w/ perso, w/o hist\\
& 15.69\% & 16.31\% & 42.81\% & 40.87\% & 9.03\% & 8.81\% & 28.69\% & 33.54\% & w/ both, w/ hist
\\ %GridSearchRH_D/LSTM1000_1110100000110Deep64_32_32_32_relu_DropOut0.65_0.22_decay0.002_lr0.00084both
& 15.92\% & 16.36\% & 42.15\% & 40.27\% & 8.84\% & 8.64\% & 29.26\% & 33.37\% & late fus SVM-D
\\
& 15.67\% & 16.33\% & 42.83\% & 40.89\% & 8.99\% & 8.84\% & 28.41\% & 33.48\% & w/ both, w/o hist
\\ 

PHD-CAD: %& 15.41\% & 16.29\% & 43.49\% & 41.93\% & 8.62\% & 8.52\% & 28.10\% & 32.84\% & w/ small perso w/ history\\%GridSearchCAD/conc0001000000110Deep128_relu_DropOut0.77_0.25_decay0.047_lr0.00012perso /-5027
%& 15.30\% & 16.21\% & 42.69\% & 40.97\% & 8.84\% & 8.68\% & 28.91\% & 33.70\% &w/ perso w/ hist\\%model?? same as above?
%& 15.37\% & 16.00\% & 43.88\% & 41.73\% & 8.53\% & 8.62\% & 27.72\% & 33.81\% & w/ perso w/o history\\
& 15.29\% & 16.15\% & 43.04\% & 41.30\% & 8.55\% & 8.63\% & 28.14\% & 33.10\% & w/ perso, w/ hist
\\%GridSearchCAD/conc0001000000110Deep512_64_relu_DropOut0.64_0.25_decay0.017_lr0.00099perso /-10183
& 15.68\% & 16.30\% & 42.53\% & 40.69\% & 8.58\% & 8.65\% & 29.28\% & 33.53\% & CAD + SVM-Dall \\

& 14.88\% & 15.61\% & 44.99\% & 43.34\% & 8.23\% & 8.14\% & 26.12\% & 31.10\% & w/ perso, w/o hist
\\
& 15.81\% & 16.50\% & 42.51\% & 40.33\% & 8.93\% & 8.92\% & 29.76\% & 34.63\% & w/ both, w/ hist\\ %GridSearchCAD/conc0001000000110Deep256_32_relu_DropOut0.62_0.17_decay0.001_lr0.00058both /-4792
& 15.96\% & 16.55\% & 41.96\% & 40.01\% & 9.09\% & 8.89\% & 30.69\% & 34.39\% & CAD + SVM-Dall
\\
& 15.59\% & 16.14\% & 43.05\% & 41.02\% & 8.76\% & 8.86\% & 28.75\% & 33.92\% & w/ both, w/o hist
\\

\hline
\multicolumn{10}{c}{The following models are trained with all perso data and a small neat DB:}\\
PHD-CAD: %& 15.76\% & 16.46\% & 42.61\% & 40.33\% & 8.94\% & 8.79\% & 30.81\% & 34.30\% & w/ both w/ hist\\%GridSearchCAD/conc0001000000110Deep128_64_relu_DropOut0.71_0.34_decay0.005_lr0.00063both /-6398
& 15.70\% & 16.37\% & 42.24\% & 40.50\% & 8.80\% & 9.00\% & 29.65\% & 34.94\% &
w/ both w/ hist, 20\\
& 15.81\% & 16.25\% & 41.88\% & 40.22\% & 8.91\% & 8.90\% & 29.83\% & 34.54\% & w/ both, w/o hist
\\
PHD-CA\_D & 15.93\% & 16.31\% & 42.05\% & 40.51\% & 9.23\% & 8.73\% & 30.28\% & 33.50\% & w/both, w/ hist, 20
\\%GridSearchCA_D/conc0011000000110Deep256_128_relu_DropOut0.77_0.42_decay0.005_lr0.00116bothSmall /-7312 NEAT smaller
& 15.60\% & 16.12\% & 41.87\% & 40.55\% & 8.87\% & 8.70\% & 29.39\% & 33.31\% & same model, more neat\\
& 15.77\% & 16.30\% & 42.92\% & 41.13\% & 9.00\% & 8.62\% & 29.38\% & 32.96\% & w/ both, w/o hist\\
& 15.79\% & 16.04\% & 43.01\% & 41.02\% & 8.79\% & 8.69\% & 29.26\% & 32.93\% & same model, more neat\\
%PHD-CA\_D & 15.41\% & 16.24\% & 42.49\% & 40.72\% & 8.52\% & 8.83\% & 29.27\% & 33.25\% & w/ perso, w/ hist, 20\\ %GridSearchCA_D/conc0011000000110Deep64_relu_DropOut0.68_0.48_decay0.002_lr0.00037perso 
%& 15.14\% & 15.97\% & 44.18\% & 41.64\% & 8.38\% & 8.63\% & 28.16\% & 32.98\% & w/ perso, w/o hist\\

\multicolumn{10}{c}{The following models are trained with a smaller perso DB and a small neat DB:}\\
PHD-SA\_D & 15.36\% & 15.76\% & 42.94\% & 40.51\% & 8.74\% & 8.55\% & 28.48\% & 32.80\% & w/ both, w/hist, 20\\ %GridSearchSA_D/conv10_1011000000110Deep64_128_relu_DropOut0.69_0.48_decay0.004_lr0.00072both 
& 15.44\% & 15.91\% & 42.60\% & 40.27\% & 8.72\% & 8.53\% & 28.99\% & 32.69\% & late fus SVM-D\\
& 15.53\% & 15.61\% & 43.30\% & 40.76\% & 8.91\% & 8.43\% & 28.53\% & 32.23\% & w/ both, w/o hist.\\

& 15.40\% & 16.03\% & 42.93\% & 41.15\% & 8.63\% & 8.55\% & 28.04\% & 33.00\% & w/ perso, w/ hist, 20 \\%GridSearchSA_D/conv10_1011000000110Deep64_128_relu_DropOut0.66_0.48_decay0.002_lr0.00014perso /-2285
& 15.46\% & 16.23\% & 42.25\% & 40.85\% & 8.64\% & 8.76\% & 29.06\% & 33.30\% & late fus SVM-D
\\
& 15.37\% & 16.05\% & 42.81\% & 41.07\% & 8.63\% & 8.55\% & 28.43\% & 32.83\% & w/ perso, w/o hist\\
\end{tabular}
\vspace{-.5ex}
\caption{Preliminary Results (temporally segmented with \cite{Gygli17DeepCut} unless otherwise indicated). For mAP, P@6 and R@6, the higher the score, the better the method. For MSD, the smallest is better.}
\label{tb:methodPref2}
\end{table*}

\begin{table*}[t!]
\centering
\setlength\extrarowheight{1ex}
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}[width=\textwidth]{@{}r|cc|cc|HHcc|P{9em}@{}}
&\multicolumn{2}{c}{mAP}&\multicolumn{2}{c}{MSD}&\multicolumn{2}{c}{%Precision @6
}&\multicolumn{2}{c|}{Recall @6}&\\[-1ex]
Model & \cite{Gygli17DeepCut} & 5 sec &  \cite{Gygli17DeepCut} & 5 sec & \cite{Gygli17DeepCut} & 5 sec& \cite{Gygli17DeepCut} & 5 sec& Notes\\\hline \hline
% PHD-CAD: & 15.41\% & 16.29\% & 43.49\% & 41.93\% & 8.62\% & 8.52\% & 28.10\% & 32.84\% & w/ perso w/ history
% \\%GridSearchCAD/conc0001000000110Deep128_relu_DropOut0.77_0.25_decay0.047_lr0.00012perso /-5027
% & 14.62\% & 15.06\% & 47.93\% & 45.82\% & 8.36\% & 8.18\% & 25.98\% & 30.53\% &w/ perso w/o history\\
% & 15.30\% & 16.13\% & 42.82\% & 40.98\% & 8.74\% & 8.76\% & 28.62\% & 33.88\% & more data w/history\\
% & 15.30\% & 16.21\% & 42.69\% & 40.97\% & 8.84\% & 8.68\% & 28.91\% & 33.70\% &same, averaged 20
% \\
% & 15.30\% & 16.21\% & 42.69\% & 40.97\% & 8.84\% & 8.68\% & 28.91\% & 33.70\% &
% same, using 20 gifs\\
% & 15.37\% & 16.00\% & 43.88\% & 41.73\% & 8.53\% & 8.62\% & 27.72\% & 33.81\% & more data w/o history\\
% PHD-CAD: & 15.76\% & 16.46\% & 42.61\% & 40.33\% & 8.94\% & 8.79\% & 30.81\% & 34.30\% &
% w/ both w/ hist\\%GridSearchCAD/conc0001000000110Deep128_64_relu_DropOut0.71_0.34_decay0.005_lr0.00063both /-6398
% & 15.56\% & 16.23\% & 43.02\% & 40.99\% & 8.98\% & 8.80\% & 29.93\% & 33.75\% & w/ both w/o hist
% \\
% & 15.69\% & 16.47\% & 42.21\% & 40.37\% & 8.73\% & 8.99\% & 29.15\% & 34.97\% & more data, w/hist
% \\& 15.70\% & 16.37\% & 42.24\% & 40.50\% & 8.80\% & 9.00\% & 29.65\% & 34.94\% & same, averaged 20
% \\
% & 15.70\% & 16.37\% & 42.24\% & 40.50\% & 8.80\% & 9.00\% & 29.65\% & 34.94\% &
% same, using 20 gifs\\
% & 15.81\% & 16.25\% & 41.88\% & 40.22\% & 8.91\% & 8.90\% & 29.83\% & 34.54\% & more data, w/o hist
% \\

% PHD-CA\_D & 15.93\% & 16.31\% & 42.05\% & 40.51\% & 9.23\% & 8.73\% & 30.28\% & 33.50\% & w/both, w/ hist, 20
% \\%GridSearchCA_D/conc0011000000110Deep256_128_relu_DropOut0.77_0.42_decay0.005_lr0.00116both /-7312 NEAT smaller
% & 15.77\% & 16.30\% & 42.92\% & 41.13\% & 9.00\% & 8.62\% & 29.38\% & 32.96\% & w/ both, w/o hist\\

% PHD-CA\_D & 15.41\% & 16.24\% & 42.49\% & 40.72\% & 8.52\% & 8.83\% & 29.27\% & 33.25\% & w/ perso, w/ hist, 20\\ %GridSearchCA_D/conc0011000000110Deep64_relu_DropOut0.68_0.48_decay0.002_lr0.00037perso 
% & 15.14\% & 15.97\% & 44.18\% & 41.64\% & 8.38\% & 8.63\% & 28.16\% & 32.98\% & w/ perso, w/o hist\\

% PHD-SA\_D & 15.36\% & 15.76\% & 42.94\% & 40.51\% & 8.74\% & 8.55\% & 28.48\% & 32.80\% & w/ both, w/hist, 20\\ %GridSearchSA_D/conv10_1011000000110Deep64_128_relu_DropOut0.69_0.48_decay0.004_lr0.00072both 
% & 15.53\% & 15.61\% & 43.30\% & 40.76\% & 8.91\% & 8.43\% & 28.53\% & 32.23\% & w/ both, w/o hist.\\
% PHD-SA\_D & 15.40\% & 16.03\% & 42.93\% & 41.15\% & 8.63\% & 8.55\% & 28.04\% & 33.00\% & w/ perso, w/ hist, 20 \\%GridSearchSA_D/conv10_1011000000110Deep64_128_relu_DropOut0.66_0.48_decay0.002_lr0.00014perso /-2285
% & 15.37\% & 16.05\% & 42.81\% & 41.07\% & 8.63\% & 8.55\% & 28.43\% & 32.83\% & w/ perso, w/o hist\\
% \hline
PHD-RH: & 15.19\% & 16.18\% & 43.79\% & 41.33\% & 8.69\% & 8.71\% & 27.47\% & 33.57\% & w/ both w/ history \\%GridSearchRH/LSTM10_101000000010Deep256_128_relu_DropOut0.77_0.16_decay0.000_lr0.00129both /-3656
PHD-RH:& 15.21\% & 16.17\% & 43.78\% & 41.34\% & 8.69\% & 8.71\% & 27.47\% & 33.57\% & w/ both w/o history\\
PHD-RHD: & 15.09\% & 15.46\% & 44.82\% & 43.48\% & 8.53\% & 8.40\% & 27.38\% & 32.34\% &
w/ neat w/ history\\%GridSearchRHD/LSTM10_101000000110Deep128_128_selu_DropOut0.76_0.12_decay0.001_lr0.00033neat 
PHD-RHD: & 15.09\% & 15.47\% & 44.82\% & 43.45\% & 8.51\% & 8.42\% & 27.34\% & 32.38\% & w/ neat w/o history\\
PHD-RHD: & 15.14\% & 15.69\% & 44.43\% & 43.85\% & 8.43\% & 8.14\% & 25.96\% & 30.53\% &
w/ perso w/ history\\%GridSearchRHD/LSTM10_101000000110Deep128_128_selu_DropOut0.76_0.12_decay0.001_lr0.00033perso /-6855
PHD-RHD: & 15.15\% & 15.69\% & 44.41\% & 43.89\% & 8.42\% & 8.14\% & 25.95\% & 30.53\% & w/ perso w/o history\\
PHD-RHD: & 15.42\% & 16.67\% & 43.28\% & 41.31\% & 9.01\% & 8.58\% & 29.32\% & 33.48\% &w/ both w/ history\\%GridSearchRHD/LSTM10_101000000110Deep128_128_selu_DropOut0.76_0.12_decay0.001_lr0.00033both 
PHD-RHD: & 15.42\% & 16.67\% & 43.26\% & 41.31\% & 9.04\% & 8.57\% & 29.39\% & 33.34\% & w/ both w/o history\\
PHD-RD & 15.24\% & 16.37\% & 43.53\% & 41.17\% & 8.76\% & 8.67\% & 28.71\% & 33.71\% & both, w/ and w/o history same \\%GridSearchRD/LSTM10_100000000010Deep128_128_relu_DropOut0.69_0.26_decay0.005_lr0.00035both /-2742
& 15.23\% & 16.06\% & 43.90\% & 41.74\% & 8.77\% & 8.52\% & 28.03\% & 32.50\% & norm\\
& 15.21\% & 16.08\% & 43.92\% & 41.76\% & 8.77\% & 8.51\% & 28.03\% & 32.46\% & norm w/o hist

\end{tabular}
\vspace{-.5ex}
\caption{Preliminary Results (temporally segmented with \cite{Gygli17DeepCut} unless otherwise indicated). For mAP, P@6 and R@6, the higher the score, the better the method. For MSD, the smallest is better.}
\label{tb:methodPref}
\end{table*}
%-----------------------------------------------------------------------------

%-----------------------------------------------------------------------------
% \begin{table*}[t!]
% \centering
% \setlength\extrarowheight{1ex}
% \setlength{\tabcolsep}{2.5pt}
% \begin{tabular}[width=\textwidth]{@{}r|cc|cc|HHcc|p{9em}@{}}
% &\multicolumn{2}{c}{mAP}&\multicolumn{2}{c}{MSD}&\multicolumn{2}{c}{%Precision @6
% }&\multicolumn{2}{c}{Recall @6}&\\[-1ex]
% Model & \cite{Gygli17DeepCut} & 5 sec &  \cite{Gygli17DeepCut} & 5 sec & \cite{Gygli17DeepCut} & 5 sec& \cite{Gygli17DeepCut} & 5 sec& Notes\\\hline \hline
% NEAT: &16.31\% &- &42.77\%&- &10.27\%&-&29.31\%&-& \hl{Internal}\\
% Random:&13.51\%&14.14\%&50.84\%&50.93\% &8.87\%&8.76\%&21.23\%&25.10\%& -\\
% vid2gif:&13.83\%&16.72\%&53.50\%&\textbf{43.76\% }&8.50\%&9.98\%&21.24\%&31.05\%& As in \cite{gygli2016video2gif}\\ 

% SVM:&14.80\%&14.95\%&49.63\%&47.52\% &&&&& -\\
% Non-PHD: &15.72\%&16.65\%&45.20\%&43.18\%&9.86\%&10.00\%&26.65\%&31.10\%& Non-perso\\ \hline %1 Deep layer (256 neurons), 0.8DropOut In, 0.4 intermidiate DropOut, 0.0015 0.1 decay (non-personalized, lr decreased @0.5 every 4 epochs) None/conc000000000000Deep256_DropOut0.80_relu_0.40_decay0.10_lr0.00150/
% %Non-PHD: &15.98\%&16.68\%&44.58\%&43.14\%&10.04\%&10.26\%&28.18\%&32.98\%& Non-perso\\ (same as before, trained on 6903 samples instead of 6167)

% PHD-CA: &16.34\%&16.82\%&45.33\%&43.69\%&10.31\%&10.07\%&28.25\%&31.94\%& averaged hist. 1D\\%1 Deep layer (256 neurons), ~0.9DropOut, 0.001 L.Rate, ~0 Decay, averaged history: Deep256_DropOut0.80_0.40_decay0.00_lr0.00100
% %PHD-CD: &16.24\%&16.76\%&44.94\%&43.19\%&10.02\%&10.15\%&27.94\%&32.03\%& min-d, d-avg 1D\\% 1 Deep layer (256 neurons), 0.8DropOut In, 0.4 intermidiate DropOut, 0.004 L.Rate decreased by a factor 0.5 every 4 epochs (total 20), 0.05 Decay, using d_to_averaged and min_d_to_any:
% PHD-CD: &16.06\%&17.04\%&44.53\%&42.32\%&10.06\%&10.20\%&28.03\%&32.86\%& stats(d) 1D\\
% %conc000000000110Deep256_DropOut0.80_0.40_decay0.05_lr0.00150/ 21 epochs 5-4-4-4-4 @.5
% PHD-CAD: &16.26\%&16.57\%&44.22\%&42.35\%&10.38\%&10.35\%&28.83\%&32.92\%& average, stats(d) 1D\\% conc010000000110Deep256_DropOut0.80_0.40_decay0.05_lr0.00150/L.Rate decreased by a factor 0.5 every 4 epochs (total 20)

% %
% %16.18\%&\%&\%&\%&\%&\%&\%& %; MSD=44.25%;  Prec@6=10.07%; Recall@6=28.36%
% %5sec: mAP=17.15%; MSD=41.73%;  Prec@6=10.28%; Recall@6=32.65%

% PHD-CW: &16.09\%&17.10\%&44.33\%&42.65\%&9.86\%&10.11\%&28.25\%&32.69\%&data * averaged hist.\\
% %conc000010000010Deep128_DropOut0.80_0.40_decay0.05_lr0.00150/
% PHD-CWD: &\textbf{16.50\%} & 16.76\% & 44.82\%& 43.04\%&10.11\%&10.11\%&28.38\%&32.02\%& data * averaged hist., stats. distances 1D \\ 
% %Deep32_DropOut0.80_0.40_decay0.05_lr0.00150 (With learning rate decreased by a factor 0.6 every 4 epochs (total 16), using `data*averaged_history`, `stats d_to_all`) Deep256_DropOut0.60_0.40_decay0.00_lr0.00300
% \hline
% PHD-SC: &16.22\%&16.67\%&44.68\%&43.46\%&10.04\%&10.00\%&28.01\%&31.73\%& 5 closest on conv \\\hline
% %conv10-1Deep64_DropOut0.80_0.40_decay0.05_lr0.00150
% PHD-RC: &16.06\%&16.73\%&44.72\%&42.99\%&9.87\%&10.14\%&27.96\%&32.11\%& 5 closest on LSTM \\
% %LSTM5Deep128_DropOut0.80_0.50_decay0.05_lr0.00150, 
% PHD-RCD: &16.23\%&16.77\%&44.76\%&42.40\%&10.02\%&10.15\%&27.98\%&32.42\%& 5 closest and dist \\
% %LSTMunnorm/LSTM10Deep128_DropOut0.80_0.40_decay0.10_lr0.00300/


% \end{tabular}
% \vspace{-.5ex}
% \caption{Preliminary Results (temporally segmented with \cite{Gygli17DeepCut} unless otherwise indicated). For mAP, P@6 and R@6, the higher the score, the better the method. For MSD, the smallest is better FOR 972 VIDEOS!!.}
% \label{tb:methodPref}
% \end{table*}
%-----------------------------------------------------------------------------


